Geometry of the Loss Landscape in Overparameterized Neural Networks: Symmetries and Invariances

We study how permutation symmetries in overparameterized multi-layer neural networks generate `symmetry-induced' critical points. Assuming a network with $ L $ layers of minimal widths $ r_1^*, \ldots, r_{L-1}^* $ reaches a zero-loss minimum at $ r_1^*! \cdots r_{L-1}^*! $ isolated points that are permutations of one another, we show that adding one extra neuron to each layer is sufficient to connect all these previously discrete minima into a single manifold. For a two-layer overparameterized network of width $ r^*+ h =: m $ we explicitly describe the manifold of global minima: it consists of $ T(r^*, m) $ affine subspaces of dimension at least $ h $ that are connected to one another. For a network of width $m$, we identify the number $G(r,m)$ of affine subspaces containing only symmetry-induced critical points that are related to the critical points of a smaller network of width $r<r^*$. Via a combinatorial analysis, we derive closed-form formulas for $ T $ and $ G $ and show that the number of symmetry-induced critical subspaces dominates the number of affine subspaces forming the global minima manifold in the mildly overparameterized regime (small $ h $) and vice versa in the vastly overparameterized regime ($h \gg r^*$). Our results provide new insights into the minimization of the non-convex loss function of overparameterized neural networks.

==> introduction.tex <==
\section*{Abstract}
We study how permutation symmetries in overparameterized multi-layer neural
networks generate `symmetry-induced' critical points.
Assuming a network with $ L $ layers of minimal widths $ r_1^*, \ldots, r_{L-1}^* $ reaches a zero-loss minimum at $ r_1^*! \cdots r_{L-1}^*! $ isolated points that are permutations of one another, %unique (up to permutation) zero-loss minimum on some learning task, 
we show that adding one extra neuron to each layer is sufficient to make all these   previously discrete minima connected into a single manifold.
For a two-layer overparameterized network of width $ r^*+ h =: m $ we explicitly describe the manifold of global minimum: it consists of $ T(r^*, m) $ affine subspaces of dimension at least $ h $ that are connected to one another.
For a network of width $m$, we identify the number $G(r,m)$ of affine subspaces containing only symmetry-induced critical points that are related to critical points of a smaller network of width $r<r^*$.
Via a combinatorial analysis, we derive closed-form formulas for $ T $ and $ G $ and show that the number $G$ of symmetry-induced critical subspaces dominates the number $T$ of affine subspaces that form the global minima manifold in the mildly overparameterized regime (small $ h $) and vice versa in the vastly overparameterized regime ($h \gg r^*$).

\section{Introduction}

Neural network landscapes are traditionally thought of as highly non-convex where non-global critical points harm gradient-descent by slowing it down (due to saddles) or making it stop in local minima.
Earlier works have argued in favor of a proliferation of saddles in high-dimensional neural network landscapes through an analogy with random error functions \cite{dauphin2014identifying}. 
On the other hand, practical neural network landscapes are found to exhibit surprising properties like the connectivity of  global minima \cite{draxler2018essentially, garipov2018loss} and convergence to a global minimum with overparameterization \cite{jacot2018neural}, ruling out proliferating saddles as a problem in this regime.
Yet, in mildly overparameterized networks, gradient descent may find a global minimum only for a small fraction of random initializations \cite{sagun2014explorations, chizat2018global, frankle2018lottery}.

In this work, we study the width-dependent scaling of the number of symmetry-induced critical points and the connectivity of global minima by exploiting the permutation symmetry and further invariances of the network parameterization. The permutation symmetry introduces an invariance against a permutation in parameterization that is characteristic for many machine learning models beyond neural networks, such as mixture models, multiple kernel learning, or matrix factorization.

Further invariances in a neural network of width $m$ induce equal loss manifolds such that all points in the manifold are equivalent to a single point in a narrower network of width $ r < m $.
The mapping approach from a point in parameter space of the narrower network to a parameter manifold  of the full network is particularly useful for the study of critical points as these critical points turn into symmetry-induced critical subspaces, and in particular, a global minimum turns into global minima subspaces that are connected to one another. % in the senses mapping that they implement the exactly the same  function mapping network inputs to outputs.

\begin{figure*}[t!]
    \input{figures/fig1}
    \vspace{-0.35cm}
    \caption{\textit{\textbf{(a-b-d)} Network representation of symmetry-induced critical points, and \textbf{(c-e)} convergence results for mildly (blue) and vastly (red) overparameterized networks for one or three hidden layers; $50$ random initializations for each network.}
     \textbf{(c)} One hidden layer student performances learning a teacher with width $ 4 $. Mildly overparameterized networks (blue) find a global minimum only for a fraction of initializations, whereas vastly overparameterized networks (red) find a global minimum for all initializations. 
    \textbf{(c)} Three hidden layer student performances learning a teacher with widths $ 4-4-4 $. Mildly overparameterized networks (blue) cannot find a global minimum despite sufficient expressivity for any of initializations, whereas vastly overparameterized networks (red) find a global minimum for all initializations. \label{fig:converge-or-not}
    }
\end{figure*}

\subsection{Main Contributions}
\begin{enumerate}
    \item Abstracting the permutation-symmetry property of (Artificial) Neural Network (NN) landscapes, we introduce the concept of replicant regions to characterize the geometry of the symmetric loss landscapes.
    \item Suppose an $ L $-layer ANN  with widths $ r_1^*, \ldots, r_{L-1}^* $ reaches a unique (up to permutation) zero-loss global minimum (we call such a network \emph{minimal} in the sense that it cannot achieve zero loss if any neuron is removed). The permutation symmetries give rise to $ r_1^*! \cdots r_{L-1}^*! $ equivalent discrete global minima.
    We show that adding one neuron to each layer is sufficient to connect these global minima into a single zero-loss manifold. 
    \item In particular, in a two-layer overparameterized network of width $ m = r^* + h $,
   we describe the geometry of the global minima manifold precisely: 
   it consists of a union of a number $ T(r^*, m ) $ of affine subspaces of dimension $ \geq h $ and it is connected.
   Furthermore, we show that the global minima manifold contains \textit{all} zero-loss points for certain smooth activation functions satisfying a condition on the derivatives at $ 0 $ and in the presence of infinitely many data points with full support of the input space. 
    \item 
    The symmetries of the network generate symmetry-induced critical points, such as saddle points, which may prevent the convergence to a global minimum (see Figure~\ref{fig:converge-or-not}). We find a surprising scaling relation between the number of subspaces formed by the symmetry-induced critical points and the number of subspaces making up the global minima:
\begin{itemize}
\item When $h\ll r^* $ (i.e. at the beginning of the overparameterized regime), the number of subspaces that make up the global minima manifold is much {\em smaller} than the number of subspaces that make up the symmetry-induced critical points. 
In this sense, there is a proliferation of saddles and the global minima manifold is `tiny'.
\item Conversely, when the number of additional neurons satisfies $h\gg r^*$ (i.e. we are far in the overparameterized regime), the number of subspaces  that make up the global minima manifold is much {\em larger} than the number of subspaces that make up the symmetry-induced (non-global) critical points. In this sense the global minima manifold is `huge'.
\end{itemize}
\item One may worry that, by adding $ h $ neurons, a saddle of a network of width $ r $ could transform into a local minimum. However, we show that this is not the case and a saddle point in the smaller network transforms into symmetry-induced saddle points in a network of width $ m $.
\end{enumerate}


\subsection{Related Work}

A number of recent works explored the typical path taken by a gradient-based optimizer.
In very wide ANNs, the gradient flow converges to a global minimum despite the non-convexity of the loss \cite{jacot2018neural, du2018gradient, chizat2018global, arora2019fine, du2019gradient, lee2019wide, lee2020finite}. %empirical investigations verify the convergence in wide enough networks
First-order gradient algorithms provably escape strict saddles \cite{jin2017escape, lee2019first};
%A gradient descent algorithm with occasional perturbation provably escapes strict saddles \cite{jin2017escape} 
however these methods can face an exponential slowdown around these saddles \cite{du2017gradient}. %pass an exponential time around these, causing a slow-down of training dynamics.
In pruned ANNs, the training with typical (random) initialization does not reach any global minimum, despite the presence of such points in the landscape \cite{frankle2018lottery}.

Another body of work focuses on identifying 
properties of neural network landscapes. The authors of \cite{dauphin2014identifying} suggested 
a proliferation of saddles in ANN landscapes through an analogy with high-dimensional Gaussian Processes. 
Other models have been proposed to understand the general structure of ANN landscapes inspired by statistical physics \cite{geiger2019jamming}, and via high-dimensional wedges \cite{fort2019large}.
These model-based empirical works focus mainly on the spectrum of critical points 
and the existence of local minima.

Another line of work suggests that SGD-found global minima are connected (i.e. there is a path linking arbitrary two minima along which the loss increases only negligibly) via simple low-loss curves \cite{draxler2018essentially, garipov2018loss}
or line segments \cite{sagun2017empirical, frankle2020linear, fort2020deep}.
Theoretical work limited to ReLU-type activation functions, showed that in overparameterized networks, all global minima lie in a connected manifold   \cite{freeman2016topology, nguyen2019connected}; note however that no geometrical description of this manifold is given. \citet{cooper2020critical} identified the geometry for a subset of the manifolds of critical points.
%Similar to our contribution regarding connectedness of the global minima, 
\citet{kuditipudi2019explaining} show that the global minima for ReLU networks, for which {\em half}  of the neurons can be dropped without incurring a significant increase in loss, are connected via piecewise linear paths of minimal cost - whereas we show that adding or removing a {\em single} neuron radically changes the connectedness without any change in loss. We are the first to prove the connectivity of the global minima manifold for continuously differentiable activation functions. 

The focus on symmetries in our work is similar to that of \cite{fukumizu2000local, brea2019weight, fukumizu2019semi} regarding the critical points coming from neuron replications. In an orthogonal direction, \citet{kunin2020neural} present a catalog of symmetries appearing in deep networks, except for the permutation-symmetry. 
In this work, we are the first to study the scaling of the number of critical points in ANN landscapes as a function of the overparameterization amount. %We find that the saddle points dominate the global minima at the onset of the overparameterization regime, whereas the global minima dominate the saddle points in the vast overparameterization regime.  
The theory presented here is challenging due to the numerous 
equivalent 
arrangements of neurons inside the network.
\newline\newline
\textbf{Notation.} For $ m \geq 1$, set $ [m] = \{ 1, \ldots, m \} $ and let $ S_m $ denote the symmetric group on $ m $ symbols, i.e. the set of permutations of $[m]$. 
For a  permutation $\pi \in S_m$ and $ D \geq 1$, the map $ \Perm_{\pi} : \R^{Dm} \to \R^{Dm} $ permutes the units $ \vartheta_i \in \R^D $ of a point $ \ptheta = (\vartheta_1, \ldots, \vartheta_m) $ according to $\pi$, i.e. $ \Perm_{\pi} \ptheta = (\vartheta_{\pi(1)}, \ldots, \vartheta_{\pi(m)}) $; we sometimes use $ \ptheta_\pi := \Perm_\pi \ptheta $.
